Dynamic Race Detection With O(1) Samples

Happens before-based dynamic analysis is the go-to technique for detecting data races in large scale software projects due to the absence of false positive reports. However, such analyses are expensive since they employ expensive vector clock updates at each event, rendering them usable only for in-house testing. In this paper, we present a sampling-based, randomized race detector that processes only constantly many events of the input trace even in the worst case. This is the first sub-linear time (i.e., running in o(n) time where n is the length of the trace) dynamic race detection algorithm; previous sampling based approaches like Pacer run in linear time (i.e., O(n)). Our algorithm is a property tester for HB-race detection -- it is sound in that it never reports any false positive, and on traces that are far, with respect to hamming distance, from any race-free trace, the algorithm detects an HB-race with high probability. Our experimental evaluation of the algorithm and its comparison with state-of-the-art deterministic and sampling based race detectors shows that the algorithm does indeed have significantly low running time, and detects races quite often.

==> exec_macros.tex <==
%!TEX root = main.tex

% Drawing executions. Arguments: # of threads, and execution.
\newcommand{\execution}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.5*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.5+1.3,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.5+1.3,0) -- (#1*1.5+1.3,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.5+1.3,-0.4*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figev}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.5 + 0.45,-0.4*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


\newcommand{\executionlarge}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.9*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.9+1.9,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.9+1.9,0) -- (#1*1.9+1.9,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.9+1.9,-0.4*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figevlarge}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.9 + 0.45,-0.4*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


% \figev arguments: thread id, event, variable/lock, 3rd arg = event id offset

% \newcommand{\mathresult}[1]{\pgfmathparse{#1} \pgfmathresult}
% \newcommand{\addmathresult}[1]{\pgfmathparse{2 *\mathresult{#1}} \pgfmathresult}

\newcommand{\figevoffset}[3]{
\pgfmathparse{#1}
\pgfmathsetmacro{\offset}{\pgfmathresult};
\pgfmathparse{\y+\offset}
\pgfmathsetmacro{\newindex}{\pgfmathresult};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\newindex}};%
\node at (#2*1.5 + 0.45,-0.4*\y) {$ #3 $};%
\pgfmathsetmacro{\y}{\y+1};
}


%\orderedeg{t1}{ind1}{off1}{t2}{ind2}{off2} denotes an edge from an event e1
% to an event e2 such that ei appears at indi in the trace and belongs to thread ti.
% off1 and off2 are offsets from the center.
\newcommand{\orderedge}[6]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] (#4*1.5 + 0.45 + #6, -0.4*#5);
}

% The 7th arg is the label and the 8th argument is the position
\newcommand{\orderedgewithlabel}[8]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] node[anchor=center, sloped, #8] { #7} (#4*1.5 + 0.45 + #6, -0.4*#5);
}

\newcommand{\executionnonumber}[2]{\begin{tikzpicture}%
                             \foreach \x in {1,...,#1}
                               \node[right] at (2*\x+0.5,0.25) {$t_{\x}$};
                             \draw (1.9,0) -- (#1*2+1.6,0);%
                             \pgfmathsetmacro{\z}{1};%
                             #2%
                             \draw (1.9,0) -- (1.9,-0.5*\z);%
                             \draw (#1*2+1.6,0) -- (#1*2+1.6,-0.5*\z);%
                             \foreach \x in {2,...,#1}
                               \draw (2*\x-0.3,0) -- (2*\x-0.3,-0.5*\z);%
                             \draw (1.9,-0.5*\z) -- (#1*2+1.6,-0.5*\z);%
                           \end{tikzpicture}}                    

\newcommand{\figevnonumber}[2]{\node [left] at (1.75,-0.4*\z) {};%
\node [right] at (#1*2 + 0.3,-0.5*\z) {$ #2 $};%
\pgfmathsetmacro{\z}{\z+1};}

% Drawing programs. Arguments: # of threads, and program
\newcommand{\figprogram}[2]{\begin{tikzpicture}%
                              \foreach \x in {1,...,#1}
                                \node at (2.3*\x-1.15,0.25) {$t_{\x}$};
                              \draw (0,0) -- (#1*2.3+0.6,0);% 
                              \pgfmathsetmacro{\y}{1};%
                              #2%
                              \draw (0,0) -- (0,-0.4*\y);% 
                              \draw (#1*2.3+0.6,0) -- (#1*2.3+0.6,-0.4*\y);% 
                              \draw (0,-0.4*\y) -- (#1*2.3+0.6,-0.4*\y);% 
                            \end{tikzpicture}}
% figstmt arguments: thread id, offset, statement
\newcommand{\figstmt}[3]{\node [left] at (-0.15,-0.4*\y) {\pgfmathprintnumber{\y}};%
                      \node[right] at (#1*2.3 + #2*0.3 - 2.15,-0.4*\y) {\texttt{#3}};
                      \pgfmathsetmacro{\y}{\y+1};}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newtheorem{observation}{Observation}

\newcommand{\nil}{\texttt{nil}}

\newcommand{\drawarrow}{\raisebox{2pt}{\scalebox{0.7}{\tikz{ \draw[-{Latex[length=2mm, width=2mm]},  ->,>=stealth](0,0) -- (7mm,0);} }}}

==> macros.tex <==
%!TEX root = main.tex

\makeatletter
\newcommand{\pnrelbar}{%
\linethickness{\dimen2}%
\sbox\z@{$\m@th\prec$}%
\dimen@=1.1\ht\z@
\begin{picture}(\dimen@,.4ex)
\roundcap
\put(0,.2ex){\line(1,0){\dimen@}}
\put(\dimexpr 0.5\dimen@-.2ex\relax,0){\line(1,1){.4ex}}
\end{picture}%
}

\newcommand{\precneq}{\mathrel{\vcenter{\hbox{\text{\prec@neq}}}}}
\newcommand{\prec@neq}{%
\dimen2=\f@size\dimexpr.04pt\relax
\oalign{%
\noalign{\kern\dimexpr.2ex-.5\dimen2\relax}
$\m@th\prec$\cr
\noalign{\kern-.5\dimen2}
\hidewidth\pnrelbar\hidewidth\cr
}%
}
\makeatother

\newenvironment{myparagraph}[1]{\noindent{\bf #1.}}{}

\newcommand{\rmv}[1] {}

% \SetInd{0.3em}{0.2em}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
% \newtheorem{observation}{Observation}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}


% Labels and references
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\problabel}[1]{\label{prob:#1}}
\newcommand{\probref}[1]{Problem~\ref{prob:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\itmlabel}[1]{\label{itm:#1}}
\newcommand{\itmref}[1]{\ref{itm:#1}}
\newcommand{\equlabel}[1]{\label{eq:#1}}
\newcommand{\equref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
% \newcommand{\appref}[1]{ the Appendix}
\newcommand{\algolabel}[1]{\label{app:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{app:#1}}
\newcommand{\linelabel}[1]{\label{line:#1}}
\newcommand{\lineref}[1]{Line~\ref{line:#1}}
\newcommand{\linerangeref}[2]{Lines~\ref{line:#1}-\ref{line:#2}}
\newcommand{\secrangeref}[2]{Sections~\ref{sec:#1}-\ref{sec:#2}}

\newcommand{\s}[1] {\mathsf{#1}}

\newcommand{\threads}[1]{\mathsf{Threads}_{#1}}
\newcommand{\locks}[1]{\mathsf{Locks}_{#1}}
\newcommand{\vars}[1]{\mathsf{Mem}_{#1}}
\newcommand{\events}[1]{\mathsf{Events}_{#1}}
\newcommand{\reads}[1]{\mathsf{Reads}_{#1}}
\newcommand{\writes}[1]{\mathsf{Writes}_{#1}}
\newcommand{\accesses}[1]{\mathsf{Accesses}_{#1}}
\newcommand{\acquires}[1]{\mathsf{Acquires}_{#1}}
\newcommand{\releases}[1]{\mathsf{Releases}_{#1}}
\newcommand{\forks}[1]{\mathsf{Forks}_{#1}}
\newcommand{\joins}[1]{\mathsf{Joins}_{#1}}
\newcommand{\match}[1]{\mathsf{match}_{#1}}
\newcommand{\lheld}[1]{\mathsf{locksHeld}_{#1}}

\newcommand{\acq}{\mathtt{acq}}
\newcommand{\rel}{\mathtt{rel}}
\newcommand{\rd}{\mathtt{r}}
\newcommand{\wt}{\mathtt{w}}
\newcommand{\fork}{\mathtt{fork}}
\newcommand{\join}{\mathtt{join}}

\newcommand{\sync}{\mathtt{sync}}
\newcommand{\lk}{\ell}
\newcommand{\ev}[1]{\langle #1\rangle}
\newcommand{\tr}{\sigma}
\newcommand{\conf}{\asymp}
\newcommand{\comp}{\circ}

\newcommand{\ThreadOf}[1]{\mathsf{thr}(#1)}
\newcommand{\OpOf}[1]{\mathsf{op}(#1)}
\newcommand{\crit}[1]{\mathsf{CS}_{#1}}

%%%%%% substring etc. %%%%%%%%%

\newcommand{\ith}[2] {#1[#2]}
\newcommand{\substr}[3] {#1[#2,#3]}
\newcommand{\prefix}[2] {\substr{#1}{0}{#2}}
\newcommand{\suffix}[2] {\substr{#1}{#2}{\infty}}
% \newcommand{\concat}{\circ}
\newcommand{\concat}{}

\newcommand{\delequal}{\triangleq}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\setpred}[2]{\{#1 \,|\, #2\}}
\newcommand{\tuple}[1]{\langle #1 \rangle}

\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
<5> <6> <7> <8> <9> <10> gen * mathb
<10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
}{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
% \DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"88}
% \DeclareMathSymbol{\varsqsubsetneq} {3}{mathb}{"8A}
% \DeclareMathSymbol{\varsqsubsetneqq}{3}{mathb}{"92}
\DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"8A}

%% Acronyms
\newcommand{\acrtr}{\textsf{tr}\xspace}
\newcommand{\acrto}{\textsf{TO}\xspace}
\newcommand{\acrhb}{\textsf{HB}\xspace}
\newcommand{\acrshb}{\textsf{SHB}\xspace}
\newcommand{\acrfhb}{\textsf{FHB}\xspace}
\newcommand{\acrchb}{\textsf{CHB}\xspace}
\newcommand{\acrcp}{\textsf{CP}\xspace}
\newcommand{\acrwcp}{\textsf{WCP}\xspace}
\newcommand{\acrsdp}{\textsf{SDP}\xspace}
\newcommand{\acrdc}{\textsf{DC}\xspace}

\newcommand{\ord}[2]{\leq^{#1}_{\mathsf{#2}}}
\newcommand{\notord}[2]{\not\leq^{#1}_{\mathsf{#2}}}
\newcommand{\strictord}[2]{<^{#1}_{\mathsf{#2}}}

\newcommand{\trord}[1]{\ord{#1}{\acrtr}}
\newcommand{\stricttrord}[1]{\strictord{#1}{\acrtr}}
\newcommand{\tho}[1]{\ord{#1}{\acrto}}
\newcommand{\stricttho}[1]{<^{#1}_{\acrto}}
\newcommand{\nottho}[1]{\not\leq^{#1}_{\acrto}}
\newcommand{\hb}[1]{\ord{#1}{\acrhb}}
\newcommand{\stricthb}[1]{\strictord{#1}{\acrhb}}
\newcommand{\notstricthb}[1]{\not<^{#1}_{\acrhb}}


\newcommand{\lw}[1]{\mathsf{lw}_{#1}}
\newcommand{\proj}[2]{#1|_{#2}}

\newcommand{\ucomment}[1]{\textcolor{red}{#1}}
\newcommand\mycommfont[1]{\ttfamily{#1}}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}

\newcommand{\cre}{\mathsf{CR}}

\renewcommand{\emptyset}{\varnothing}

\input{exec_macros}
\input{pseudocode_macros}


\newcommand{\nats}{\mathbb{N}}
\newcommand{\rapid}{\textsf{RAPID}\xspace}
\newcommand{\pacer}{\textsc{Pacer}\xspace}
\newcommand{\RND}{{\bf\textsf{RPT}}\xspace}
\newcommand{\pe}{\textsc{processed event}\xspace}
\newcommand{\raciness}{\text{raciness}\xspace}
\newcommand{\samplecost}{\textsc{sample cost}\xspace}
\newcommand{\cost}{\textsc{analysis cost}\xspace}


\newcommand{\djit}{\textsc{Djit}\xspace}
\newcommand{\djitp}{\textsc{Djit}+\xspace}
\newcommand{\fasttrack}{\textsc{FastTrack}\xspace}
\newcommand{\eraser}{\textsc{Eraser}\xspace}
\newcommand{\tsan}{\textsc{ThreadSanitizer}\xspace}

\newcommand{\vc}[1]{$\langle${\texttt{#1}}$\rangle$}

%% Table

\newcommand\VRule[1][\arrayrulewidth]{\vrule width #1}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

%%%

%%%%%%%%%% Macros for property tester %%%%%%%%

\newcommand{\hamd} {d_{\s{h}}}
\newcommand{\numsam} {r}
\newcommand{\samlen} {k}
\newcommand{\lh} {h}
\newcommand{\rcf} {\s{RF}}


%%%%%%%%%% Trace numbers %%%%%%%%%%
\newcounter{count}

\newcommand\generator[1]%
{%
  \stepcounter{count}%
  \expandafter\edef\csname#1\endcsname{\thecount}%
}

\generator{one}
\generator{two}
\generator{three}
\generator{four}
\generator{five}
\generator{six}




==> pseudocode_macros.tex <==
%!TEX root = ./main.tex

%%%%%% Macros for algo %%%%%%%%
\SetKwProg{myfun}{function}{}{}
\SetKwProg{myhandler}{handler}{}{}
\SetKwFunction{init}{InitMetadata}
\SetKwFunction{reset}{resetData}
\SetKwFunction{checkAndUpdate}{checkRaceAndUpdateMetadata}
\SetKwFunction{merge}{mergeSubtraces}
% \SetKwFunction{fixpoint}{ComputeLCClosure}
\SetKwFunction{fixpoint}{ComputeSPIdeal}
\SetKwFunction{maxLB}{maxLowerBound}
\SetKwFunction{checkRace}{checkRace}
\SetKwFunction{rdhandler}{read}
\SetKwFunction{wthandler}{write}
\SetKwFunction{acqhandler}{acquire}
\SetKwFunction{relhandler}{release}
\SetKwInput{Params}{Parameters}
\SetKwInput{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{Let}{let}
\SetKw{Break}{break}
\SetKw{NOT}{not}
\SetKw{declare}{declare}
\SetKw{check}{check}
\SetKw{exit}{exit}
\SetKwFor{Foreach}{for each}{}{}%
\DontPrintSemicolon
% \newcommand{\ideal}{\mathsf{I}}
\renewcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}

% \newcommand{\gets}{\leftarrow}

\newcommand{\AcqLst}{\mathsf{CSHist}}
\newcommand{\AccLst}{\mathsf{AccessHist}}

\newcommand{\mx}{\sqcup}
\newcommand{\cle}{\sqsubseteq}
\newcommand{\Cc}{\mathbb{C}}
\newcommand{\Ll}{\mathbb{L}}
\newcommand{\Rr}{\mathbb{R}}
\newcommand{\Ww}{\mathbb{W}}
\newcommand{\LW}{\mathbb{LW}}
\newcommand{\Ii}{\mathbb{I}}
\newcommand{\gId}{\mathbbm{g}}
\newcommand{\lastGID}{\gId\mathsf{\_max}}
\newcommand{\lastRelTime}{\mathsf{RelTime\_max}}

\newcommand{\view}[3]{{#1}_{#2}^{#3}}

\renewcommand{\nil}{\mathtt{NIL}}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother
\newcommand{\apicall}[3]{{#1}\bigcdot{\textup{\texttt{#2(#3)}}}}
\newcommand{\first}[1]{\apicall{#1}{first}{}}
\newcommand{\removeFirst}[1]{\apicall{#1}{removeFirst}{}}
\newcommand{\isEmpty}[1]{\apicall{#1}{isEmpty}{}}
\newcommand{\lst}[1]{\apicall{#1}{last}{}}
\newcommand{\addLst}[2]{\apicall{#1}{addLast}{#2}}
\newcommand{\updateRel}[2]{\apicall{#1}{updateRelease}{#2}}

\newcommand{\true}{\top\!\!\!\!\top}
\newcommand{\false}{\bot\!\!\!\!\bot}

